Novel techniques for efficient quantum state tomography and quantum process tomography and their experimental implementation

This thesis actively focuses on designing, analyzing, and experimentally implementing various QST and QPT protocols using an NMR ensemble quantum processor and superconducting qubit-based IBM cloud quantum processor. Part of the thesis also includes a study of duality quantum simulation algorithms and Sz-Nagy's dilation algorithm on NMR where several 2-qubit non-unitary quantum channels were simulated using only a single ancilla qubit. The work carried out in the thesis mainly addresses several important issues in experimental QST and QPT which include: i) dealing with invalid experimental density (process) matrices using constraint convex optimization (CCO) method, ii) scalable QST and QPT using incomplete measurements via compressed sensing (CS) algorithm and artificial neural network (ANN) technique, iii) selective and direct measurement of unknown quantum states and processes using the concept of quantum 2-design states and weak measurement (WM) approach and iv) quantum simulation and characterization of open quantum dynamics using the dilation technique.

==> abbreviation.tex <==
\chapter{Abbreviations used in the Thesis}
%\vspace{-8cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[H]
\begin{center}
%\caption{}
\begin{tabular}{l l l }%{lcdr}
%\hline
BE    &:& Bound Entangled \\
BS    &:& Bi-Separable \\
CCNR  &:& Computable Cross Norm or Realignment \\
CP    &:& Completely Positive \\
CHSH  &:& Clauser-Horne-Shimony-Holt \\
EM    &:& Entanglement Measure(s) \\
EPR   &:& Einstein-Podolsky-Rosen \\
EW    &:& Entanglement Witness \\
FID   &:& Free Induction Decay \\
FT    &:& Fourier Transform \\
GHZ   &:& Greenberger-Horne-Zeilinger \\
LOCC  &:& Local Operations and Classical Communications \\
NCC   &:& Non Classical Correlations \\
NMR   &:& Nuclear Magnetic Resonance \\
NMRQC &:& NMR Quantum Computing \\
NPT   &:& Negative under Partial Transpose \\
PCC   &:& Properly Classically Correlated \\
PNCP  &:& Positive but Not Completely Positive\\
POVM  &:& Positive Operator Valued Measure\\
PPT   &:& Positive under Partial Transpose \\
PT    &:& Partial Transposition \\
QC    &:& Quantum Computing \\
QD    &:& Quantum Discord \\
QIP   &:& Quantum Information Processing \\
QST   &:& Quantum State Tomography \\
RF    &:& Radio Frequency \\
SDP   &:& Semi Definite Program/Programming \\
SLOCC &:& Stochastic LOCC \\
%\hline
\end{tabular}
\end{center}
\end{table}
